Constrained Bayesian ICA for Brain Connectome Inference

Brain connectomics is a developing field in neurosciences which strives to understand cognitive processes and psychiatric diseases through the analysis of interactions between brain regions. However, in the high-dimensional, low-sample, and noisy regimes that typically characterize fMRI data, the recovery of such interactions remains an ongoing challenge: how can we discover patterns of co-activity between brain regions that could then be associated to cognitive processes or psychiatric disorders? In this paper, we investigate a constrained Bayesian ICA approach which, in comparison to current methods, simultaneously allows (a) the flexible integration of multiple sources of information (fMRI, DWI, anatomical, etc.), (b) an automatic and parameter-free selection of the appropriate sparsity level and number of connected submodules and (c) the provision of estimates on the uncertainty of the recovered interactions. Our experiments, both on synthetic and real-life data, validate the flexibility of our method and highlight the benefits of integrating anatomical information for connectome inference.

==> optimization.tex <==
% !TEX root = main_bayes.tex

An alternative approach would be the folloowing:
Stein loss is defined as:
$$ L(\hat{\Sigma},\Sigma) =  tr(\hat{\Sigma} \Sigma^{-1}) - \log(| \hat{\Sigma} \Sigma^{-1}|) -p$$
We use it here with $\Sigma=\frac{Y^TY}{T}$ the e,prirical correlation matrix.
We want to solve:
$$ \hat{\Sigma} = A^TA + \text{diag}(\gamma_i^2)  $$
The loss is convex as a function of $\hat{\Sigma}$ but not a a function of $A$. We thus use composite algorithm to make this more convex:
The full problem can be iteratively solved as:

\begin{equation}
    \begin{split}
        \text{Minimize }_{\hat{\Sigma}}& tr(\hat{\Sigma} \Sigma^{-1}) - \log(| \hat{\Sigma} \Sigma^{-1}|) -p\\
        \text{ such that } &  \hat{\Sigma} = A^TA + \text{diag}(\gamma_i^2)\\
        & \text{diag}(\hat{\Sigma}) = 1\\
    \end{split}{}
\end{equation}

We liearize the problem
\begin{equation}
    \begin{split}
        \text{Minimize }_{\hat{\Sigma}}& tr(\hat{\Sigma} \Sigma^{-1}) - \log(| \hat{\Sigma} \Sigma^{-1}|) -p\\
        \text{ such that } &  \hat{\Sigma} = (A^{(k)})^TA^{(k)} + 2A^{(k)}^T \delta A  + \text{diag}(\gamma_i^2)\\
        & \text{diag}(\hat{\Sigma}) = 1\\
         & || \delta A|| \leq \delta \\
         & A^{(k+1)} =  A^{(k+1)} + \delta A 
    \end{split}{}
\end{equation}
We also want to put smoothness constraints on $ A^{(k+1)}$.
This problem is now convex and we know that there exists a global optimal soliution. It might thus heavily depend on global initalization.
This way our problem is a little more solvable than it used to be.
Thus the algorithm would operate as follows:
\begin{itemize}
    \item Optimize with respect to $\delta_A$ and $\gamma$
    \item find a solution for $A^{(k+1)}$
    \item Iterate
    
\end{itemize}


